Advancing Referring Expression Segmentation Beyond Single Image

Referring Expression Segmentation (RES) is a widely explored multi-modal task, which endeavors to segment the pre-existing object within a single image with a given linguistic expression. However, in broader real-world scenarios, it is not always possible to determine if the described object exists in a specific image. Typically, we have a collection of images, some of which may contain the described objects. The current RES setting curbs its practicality in such situations. To overcome this limitation, we propose a more realistic and general setting, named Group-wise Referring Expression Segmentation (GRES), which expands RES to a collection of related images, allowing the described objects to be present in a subset of input images. To support this new setting, we introduce an elaborately compiled dataset named Grouped Referring Dataset (GRD), containing complete group-wise annotations of target objects described by given expressions. We also present a baseline method named Grouped Referring Segmenter (GRSer), which explicitly captures the language-vision and intra-group vision-vision interactions to achieve state-of-the-art results on the proposed GRES and related tasks, such as Co-Salient Object Detection and RES. Our dataset and codes will be publicly released in https://github.com/yixuan730/group-res.

==> figures/blank.tex <==
\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Example of a caption.  It is set in Roman so mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
\label{fig:long}
\label{fig:onecol}
\end{figure}

==> figures/two_col_teaser.tex <==
\twocolumn[{
  \maketitle
  \vspace{-22pt}
  \begin{center}
    \fbox{\rule{0pt}{1.6in} \rule{.95\linewidth}{0pt}}
    \vspace{-2pt}
    \captionsetup{type=figure}
    \captionof{figure}{Several applications of LOCS. XXXXXXX,XX,XXXXX
    }
  \label{fig:teaser}
  \end{center}
}]

==> figures/vis_withrawimg.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=1\linewidth]{figures/vis_withrawimg_.pdf}
\end{center}
\vskip -2 em
   \caption{\textbf{Visualizations of the prediction mask, feature maps, heatmaps, and corresponding image group} on an example from the G-RefCg test set. The leftmost column demonstrates the input image, predicted mask (in \ty{yellow}) and ground-truth mask (in \tg{green}). In the first row of other columns, we visualize the feature maps in decoder (\ie, $\mathmat{Y}_{i}$) activated by linguistic feature $\mathmat{L}$, and feature maps in decoder (\ie, $\mathmat{Y}_{i}^{anti}$) activated by linguistic anti-feature $\mathmat{L}^{anti}$ in our proposed mirror training process (Sec. 3.4 in main paper). In the second and third row, we demonstrate the language-activated heatmap $\mathmat{M}^{l}$ (the one inside the solid \tg{green} border) and vision-activated heatmaps $\mathmat{M}^{v}$ (the others inside the dotted border) . Note that the raw order of heatmaps are shown in the second row, and the well-ranked heatmaps are demonstrated in the third row. In the bottom row, we present the image group, with each image corresponding to one vision-activated heatmap. The arrows represent the one-to-one correspondence between the images and the rearranged heatmaps. 
   Best viewed in color.}
       \vspace{-7pt}
\label{fig:vis_withrawimg}
\end{figure*}
